Pion-induced radiative corrections to neutron beta-decay

We compute the electromagnetic corrections to neutron beta decay using a low-energy hadronic effective field theory. We identify and compute new radiative corrections arising from virtual pions that were missed in previous studies. The largest correction is a percent-level shift in the axial charge of the nucleon proportional to the electromagnetic part of the pion-mass splitting. Smaller corrections, comparable to anticipated experimental precision, impact the $\beta$-$\nu$ angular correlations and the $\beta$-asymmetry. We comment on implications of our results for the comparison of the experimentally measured axial charge with first-principle computations using lattice QCD and on the potential of $\beta$-decay experiments to constrain beyond-the-Standard-Model interactions.

==> decayrate.tex <==
{\it Neutron decay rate to $\mathcal O(\alpha \epsilon_\slashpi)$ --- } \\


==> lattice.tex <==
\begin{figure}
\begin{tabular}{ccc}
\raisebox{-\height}{\includegraphics[width=0.3\columnwidth]{figures/electron_structure}}&
\raisebox{-\height}{\includegraphics[width=0.3\columnwidth]{figures/nucleon_electron}}&
\raisebox{-\height}{\includegraphics[width=0.3\columnwidth]{figures/nucleon_structure}}\\
a& b& c
\end{tabular}
\caption{\label{fig:correlation_functions}
Contributions to neutron decay from three classes of diagrams described in the text.
The solid lines are the nucleons, electron and neutrino and the wiggly line is the photon.
The open boxes denote the insertion of the weak-interaction vertices.
The gray ellipse denotes the non-perturbative QCD corrections which include the radiative pion contributions, among others.
}
\end{figure}

{\it Determining the LECs in lattice QCD --- }
The perturbative nature of QED allows for a ``factorization'' of the corrections into three general diagrams, depicted in Fig.~\ref{fig:correlation_functions}:
a) The self-energy correction to the electron (including undepicted Bremsstrahlung radiation);
b) The interference ``triangle'' diagram (including Bremsstrahlung);
c) The non-perturbative nucleon structure corrections, including the elastic Born terms, the nucleon self-energy corrections (and Bremsstrahlung) as well as the radiative pion corrections determined in this work.
This last diagram represents a well defined correlation function that can be computed with lattice QCD + QED.
One natural scheme for including QED with lattice QCD calculations is QED$_{\rm M}$, in which an explicit photon mass is introduced to regulate the infrared behavior~\cite{Endres:2015gda}.
With such a setup, the lattice calculation would naturally exclude the Bremsstrahlung radiation as the photon excitation would be gapped by the photon mass, which is typically $m_\gamma/m_\pi \approx 1/2$ in QED$_{\rm M}$ calculations.
The ground state correlation function would then contain $\ln(m_\gamma)$ divergences, which could be identified and cancelled analytically, prior to taking the $m_\gamma\rightarrow0$ limit~\cite{Carrasco:2015xwa}.
{\color{blue}There are further subtleties that must be considered such as the renormalization of the quark level operators which do not factorize from the leptonic legs~cite{DiCarlo:2019knp}.
Also, diagram c) is not gauge invariant on its own, but the EFT calculation can be performed in the same gauge as the lattice calculation in which case the LECs will depend upon the gauge.}


==> pionlessEFT.tex <==

{\it $\slashpi$EFT setup for neutron decay --- } 
At the energies relevant for $\beta$ decays, we  integrate out the pion  and match onto a theory with only nucleons, photons and leptons.
This is done by taking   the large $m_\pi$ limit in the  amplitudes of order $G_F \alpha$ and  $G_F \alpha \epsilon_\chi$ 
in Figs.~\ref{Fig:DiagLO} and \ref{Fig:DiagNLO}.   This provides, consistently with the decoupling theorem, 
local amplitudes  of order $G_F  \alpha \epsilon_\chi^n \epsilon_\slashpi^0$,   $G_F \alpha \epsilon_\chi^n \epsilon_\slashpi$, ... in the low-energy pionless EFT. 
Retaining only the terms that contribute to 
%In order to capture the terms of
 $O(G_F \epsilon_{\rm recoil})$,  $O( G_F \alpha)$,  $O( G_F \alpha \epsilon_\chi)$, and  $O( G_F \alpha \epsilon_\slashpi)$, 
we include in  the pionless effective Lagrangian  the following operators of dimension six and seven
%~\footnote{We neglect here dimension-seven operators  that do not receive contributions from the $1/m_N$ expansion nor from pion loops.}
%
%\begin{eqnarray}\label{eq:Lpiless}
% \mathcal L_{\slashpi} &=& \bar N (g_V v^\mu - 2 g_A S^\mu) N \bar e \gamma_\mu P_L \nu \nonumber \\ && - \frac{i}{4 m_N} (1+\kappa_{\rm weak}) \bar N [S^\mu, %S^\nu] N\,   \partial_\nu \left(  \bar e \gamma_\mu P_L \nu \right) \nonumber \\ 
% & & +  \frac{i g_T m_e}{4 m_N} \bar N \left( S^\mu v^\nu - S^\nu v^\mu\right) N\,   \left(  \bar e \sigma_{\mu \nu} P_L \nu \right) 
%\end{eqnarray}
%
\begin{eqnarray}\label{eq:Lpiless}
 \mathcal L_{\slashpi} &=& 
 - \sqrt{2}  G_F V_{ud}  \, \bigg[
  \bar e \gamma_\mu P_L \nu_e 
   \bigg(
  \bar N  \left(g_V  v_\mu - 2 g_A  S_\mu \right)  \tau^+ N  
 \nonumber \\ 
 &+ & \frac{i}{2 m_N}  \bar N 
  (v^\mu v^\nu - g^{\mu \nu}  - 2 g_A v^\mu S^\nu) (  \overleftarrow   \partial - \overrightarrow \partial)_\nu  \tau^+ N  
  \bigg)
  %\  \bar e \gamma_\mu P_L \nu_e  
  \nonumber \\ 
 & +& 
 %- \sqrt{2} G_F V_{ud} 
 \frac{i \mu_{\rm weak}}{m_N}    \bar N [S^\mu, S^\nu]  \tau^+ N\,   \partial_\nu \left(  \bar e \gamma_\mu P_L \nu \right)
  \nonumber \\ 
% &+ & \frac{i}{2 m_N}  \bar N 
%  (v^\mu v^\nu - g^{\mu \nu}  - 2 g_A v^\mu S^\nu) (  \overleftarrow   \partial - \overrightarrow \partial)_\nu  \tau^+ N  \  \bar e \gamma_\mu P_L \nu_e  
%  \nonumber \\ 
   %- \sqrt{2} G_F V_{ud} 
&+ & 
    \frac{i c_T m_e}{m_N} \bar N \left( S^\mu v^\nu - S^\nu v^\mu\right)  \tau^+ N\,   \left(  \bar e \sigma_{\mu \nu} P_L \nu \right)  \bigg]~.
%  & & +  \frac{i g_T m_e}{4 m_N} \bar N \left( S^\mu v^\nu - S^\nu v^\mu\right)  \tau^+ N\,   \left(  \bar e \sigma_{\mu \nu} P_L \nu \right) 
\end{eqnarray}
We provide below expressions for the LECs $g_V, g_A, \mu_{\rm weak}, c_T$ in terms of 
LECs appearing in the HBChPT Lagrangian and electromagnetic loop corrections involving the pion. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%In absence of electromagnetic corrections one has  $g_V=1$ (up to second-order corrections in the quark mass difference $m_u-m_d$). 
%$g_A$ represents the isopsin-symmetric nucleon charge (related to $g_A^{(0)}$  of Eq,~(\ref{eq:L1}) by all order chiral corrections in $\epsilon_\chi^n$),    
%the weak magnetism term is determined  in terms of proton and neutron magnetic moments $\mu_{\rm weak}= \mu_p - \mu_n$, and $c_T =0$. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




